L_DMI: An Information-theoretic Noise-robust Loss Function

Accurately annotating large scale dataset is notoriously expensive both in time and in money. Although acquiring low-quality-annotated dataset can be much cheaper, it often badly damages the performance of trained models when using such dataset without particular treatment. Various methods have been proposed for learning with noisy labels. However, most methods only handle limited kinds of noise patterns, require auxiliary information or steps (e.g. , knowing or estimating the noise transition matrix), or lack theoretical justification. In this paper, we propose a novel information-theoretic loss function, $\mathcal{L}_{DMI}$, for training deep neural networks robust to label noise. The core of $\mathcal{L}_{DMI}$ is a generalized version of mutual information, termed Determinant based Mutual Information (DMI), which is not only information-monotone but also relatively invariant. \emph{To the best of our knowledge, $\mathcal{L}_{DMI}$ is the first loss function that is provably robust to instance-independent label noise, regardless of noise pattern, and it can be applied to any existing classification neural networks straightforwardly without any auxiliary information}. In addition to theoretical justification, we also empirically show that using $\mathcal{L}_{DMI}$ outperforms all other counterparts in the classification task on both image dataset and natural language dataset include Fashion-MNIST, CIFAR-10, Dogs vs. Cats, MR with a variety of synthesized noise patterns and noise amounts, as well as a real-world dataset Clothing1M. Codes are available at https://github.com/Newbeeer/L_DMI .

==> others.tex <==
\begin{definition}[Determinant Mutual Information]\label{def:dmi}
    Given two random variables $X,Y$ which have the same support $\Sigma$, we define the determinant mutual information between $X$ and $Y$ as $$DMI(X;Y)=|\det(U_{X,Y})|.$$
\end{definition}



%Note that Lemma~\ref{lem:deter2} shows that $Quality(R)\in [0,1]$ and equals 1 if and only if the reference is a permutation of ground truth, i.e. no information is lost. 

\begin{lemma}
    $DMI$ is non-negative and striclty $({\leq}^{\cdot}_t)$-monotone. Moreover, $$DMI(O;R)=|\det(T_{G,R})| DMI(O;G).$$
\end{lemma}

\begin{proof}
The non-negativity of $DMI$ follows directly from its definition. When $O'{\preccurlyeq}^G_t ({\prec}^G_t) O$, we have $|det(T_{G,O'})|\leq (<) |det(T_{G,O})|$, then
\begin{align*}
    DMI(O';G)&=|det(U_{O',G})|\\ \tag{Lemma~\ref{lem:deter1}}
             &=|det(U_{G,G})||det(T_{G,O'})|\\ 
             &\leq (<) |det(U_{G,G})||det(T_{G,O})|=DMI(O;G).
\end{align*}
Thus, $DMI$ is striclty $({\leq}^{\cdot}_t)$-monotone. Moreover, 

    \begin{align*}
        DMI(O;R) & = |\det(U_{O,R})|\\ \tag{Claim~\ref{claim:independent}}
                 & = |\det(U_{O,G}\cdot T_{G,R})|\\
                 & = |\det(T_{G,R})||\det(U_{O,G})|\\
                 & = |\det(T_{G,R})|DMI(O;G)\\
                % & =|\det(T_{G,R})|DMI(G;G)|\det(T_{G,O})|
    \end{align*}
\end{proof}

%$\frac{score_R^{DMI}(O)}{score_R^{DMI}(O')}$ is independent of $R$

The above lemma and the main theorem directly imply the following corollary. 

\begin{corollary}\label{cor:dmi}
Consider a setting $(G,R,\mathcal{O})$ where $T_{G,R}$ is invertible and every object in $\mathcal{O}$ has the same support as the ground truth $G$. $score_R^{DMI}$ is non-negative, acceptable, and strictly ${\leq}^{G}_t$-monotone. 
Moreover, for every $O\in \mathcal{O}$
    $$score_R^{DMI}(O)=|\det(T_{G,R})| score_G^{DMI}(O),$$ which implies that $score_R^{DMI}$ is ratio-reference-free.
\end{corollary}
